Specification-Aware Predictive Uncertainty Decomposition

Classical decompositions of predictive uncertainty, such as the information-theoretic one, are defined for a fixed representation $x$ of the input object. They do not consider that $x$ may be incomplete, nor do they measure how much the missing information can affect the prediction. In Large Language Models, users can clarify an underspecified input without any retraining. The clarified input can describe the user's unobserved intent $z^*$ more accurately and change the predictive uncertainty about the outcome. In this paper, we formalize this setting probabilistically and derive a three-term decomposition of prediction risk into specification, residual aleatoric, and epistemic uncertainties. We show that at the original information level, when only $x$ is available, the aleatoric uncertainty, represented by a Bayes risk, has two components. The first, which we call specification uncertainty, is the expected reduction in this Bayes risk from revealing the intent. The second is the residual aleatoric uncertainty, i.e., the Bayes risk that remains once the intent is known, averaged over its possible values $z$ given $x$. The distinction is important, as specification uncertainty informs the decision to request clarification before making a prediction. We build approximations of these components and connect them to existing uncertainty measures. Our experiments across different domains and modalities show distinct roles for the three components. Specification uncertainty is the most informative for detecting underspecified inputs, while residual aleatoric uncertainty is the most informative for detecting in-distribution prediction errors.

==> figures/language_domain/correlation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/language_domain/ensemble_gemma4_e4b_ensemble_n40_20260807_131258_se_direct_term_pairs.png}
    \caption{Correlation between components of SEA decomposition. Sample size 200: 100 well-formed (single) and 100 ambiguous (ambi) queries. Specification uncertainty is almost orthogonal to both aleatoric and epistemic terms, while they are correlated, especially on ambiguous inputs.}
    \label{fig:sea_correlation}
\end{figure}


==> figures/language_domain/ensemble_size_ablation.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/language_domain/ensemble_size_auroc_semantic_inserted.png}
    \caption{ROC-AUC as a function of ensemble size. Based on ensemble of size 4, all model subsets are evaluated: 4 single-model, 6 pairs, 4 triples and the full set.}
\label{fig:ensemble_size_text_QA}
\end{figure}


==> tables/vqa_imagenet_errord.tex <==
\begin{table}[]
    \centering
    \caption{ROC-AUC for error detection with the heterogeneous ensemble on Imagenet. Positive class is an incorrect answer to the masked image. Each entry is the unweighted mean of AUROCs over the 10\%, 20\%, 30\%, and 50\% mask levels; 500 images per level sampled from the Imagenet validation set.}
    \label{tab:vqa_imagenet_errord_granular}
    \begin{tabular}{lrrrr}
\toprule
Group & Total & Aleatoric & Epistemic & Specification \\
\midrule
\multicolumn{5}{l}{\textit{SEA decomposition}} \\
\cmidrule(lr){1-5}
SE & 0.7487 & 0.7469 & 0.7241 & 0.6640 \\
SE norm. & 0.7706 & 0.7686 & \textbf{0.7356} & 0.6708 \\
SE direct & 0.7494 & 0.7500 & 0.7177 & \textbf{0.6737} \\
SE direct norm. & 0.7423 & 0.7307 & 0.7282 & 0.6647 \\
MCSE & 0.7566 & 0.7511 & 0.7295 & 0.6635 \\
MCNSE & \textbf{0.7805} & \textbf{0.7740} & 0.7069 & 0.6701 \\
\addlinespace
\multicolumn{5}{l}{\textit{BALD (without clarifications)}} \\
\cmidrule(lr){1-5}
SE & 0.7437 & 0.7351 & 0.7168 & - \\
SE norm. & 0.7707 & 0.7648 & 0.7273 & - \\
SE direct & 0.7447 & 0.7426 & 0.7070 & - \\
SE direct norm. & 0.7434 & 0.7263 & \textbf{0.7307} & - \\
MCSE & 0.7527 & 0.7421 & 0.7227 & - \\
MCNSE & \textbf{0.7823} & \textbf{0.7717} & 0.7092 & - \\
\addlinespace
\multicolumn{5}{l}{\textit{Baselines (posterior over visual clarifications)}} \\
\cmidrule(lr){1-5}
MSP & \textbf{0.7418} & - & - & - \\
PPL & 0.7055 & - & - & - \\
MTE post. & 0.7126 & - & - & - \\
MTE unif. & 0.7171 & - & - & - \\
\addlinespace
\multicolumn{5}{l}{\textit{Baselines (without visual clarifications)}} \\
\cmidrule(lr){1-5}
MSP & \textbf{0.7505} & - & - & - \\
PPL & 0.7115 & - & - & - \\
MTE post. & 0.7095 & - & - & - \\
MTE unif. & 0.7120 & - & - & - \\
\bottomrule
\end{tabular}
\end{table}
